Self-supervised surface-related multiple suppression with multidimensional convolution

Surface-related multiples pose significant challenges in seismic data processing, often obscuring primary reflections and reducing imaging quality. Traditional methods rely on computationally expensive algorithms, the prior knowledge of subsurface model, or accurate wavelet estimation, while supervised learning approaches require clean labels, which are impractical for real data. Thus, we propose a self-supervised learning framework for surface-related multiple suppression, leveraging multi-dimensional convolution to generate multiples from the observed data and a two-stage training strategy comprising a warm-up and an iterative data refinement stage, so the network learns to remove the multiples. The framework eliminates the need for labeled data by iteratively refining predictions using multiples augmented inputs and pseudo-labels. Numerical examples demonstrate that the proposed method effectively suppresses surface-related multiples while preserving primary reflections. Migration results confirm its ability to reduce artifacts and improve imaging quality.

==> Sections/Acronyms.tex <==
\makeglossaries
\newacronym{gcd}{GCD}{Greatest Common Divisor}
\newacronym{lcm}{LCM}{Least Common Multiple}


==> Sections/Headers.tex <==
% Page headers
\pagestyle{fancy}
\fancyhf{}
\rhead{DW0085  --  01 / 04 / 2025}
% \lhead{\raisebox{-0.5\height}{\includegraphics[height=17mm]{Figures/DigLogo.eps}}}
\lhead{\raisebox{-0.5\height}{\includegraphics[height=17mm]{Figure/DeepWave.png}}}
\rfoot{P\thepage}


% Title
\title{\vspace{5mm}\fontsize{18pt}{20pt}\selectfont\textbf{Self-supervised surface-related multiple suppression with multidimensional convolution}} 

\author{
\large
\textsc{Shijun Cheng\textsuperscript{1}, Ning Wang \textsuperscript{1}, and Tariq Alkhalifah\textsuperscript{1}}\\[2mm]
\large \textsuperscript{1}King Abdullah University of Science and Technology, Thuwal, Kingdom of Saudi Arabia
%\vspace{2mm}
}
\date{}



==> Sections/Keywords.tex <==
\keywords{Surface-related multiples suppression, Multidimensional convolution, Self-supervised learning, Neural network}

==> Sections/Symbols.tex <==
\makenomenclature
\nomenclature{\(c\)}{Speed of light in a vacuum}
\nomenclature{\(h\)}{Planck constant}
